Training Transformers for KV Cache Compressibility

Long-context language modeling is increasingly constrained by the Key-Value (KV) cache, whose memory and decode-time access costs scale linearly with the prefix length. This bottleneck has motivated a range of context-compression methods, from token-level summarization to recent optimization-based KV compression methods. These post-hoc methods operate on the KV cache of a fixed pretrained model, so their effectiveness is fundamentally limited by how well the model's internal representations can be compressed. In this work, we formalize the notion of KV compressibility and show that it is a property of the learned representations, rather than of the context alone. We prove that almost any sequence-to-vector function admits both highly compressible and inherently non-compressible transformer implementations, highlighting the need to guide transformers toward compressible representations during training. Motivated by this, we propose KV-Compression Aware Training (KV-CAT), a continued pretraining procedure that incentivizes the emergence of compressible representations. We introduce a train-time KV sparsification policy that masks KV slots during training. This forces the model to use fewer KV slots and encourages it to learn representations amenable to post-hoc compression. Empirically, we show that KV-CAT improves the quality-budget tradeoff of downstream compression methods across retrieval, long-context question answering, and perplexity-based evaluation of compressed-prefix continuation.

==> sections/learning_to_compress.tex <==
\section{Training for Cache Compressibility}

As shown in the previous section, training transformers to solve sequence-to-vector tasks may admit both compressible and non-compressible solutions. That is, compressibility is not just a property of the input context itself, but of the particular representation learned by the model. This naturally raises the following question:
% \begin{insight}{Key question}
% Can we incentivize more compressible transformers during training, and if so, how?
% \end{insight}
\begin{insight}
 cCan we guide transformers towards more compressible representations during training? 
\end{insight}

To answer this question, we introduce KV-Compression Aware Routed Training (\ourmethod), a continued pre-training procedure that explicitly encourages compressible internal representations.
% We then provide empirical evidence demonstrating its effectiveness across a range of tasks, transformer sizes, and post-hoc compression methods.

\input{sections/method}
\input{sections/experiments}


==> tikz/kv_compression_policy.tex <==
\begin{tikzpicture}[
    >=Latex,
    font=\sffamily\scriptsize,
    token/.style={draw=black!72, line width=0.55pt, rounded corners=1pt, minimum width=0.34cm, minimum height=0.32cm, inner sep=1pt, align=center},
    slot/.style={draw=black!72, line width=0.6pt, rounded corners=1pt, minimum width=0.48cm, minimum height=0.38cm, inner sep=1pt, align=center},
    block/.style={draw=black!78, line width=0.75pt, rounded corners=1.5pt, minimum width=1.04cm, minimum height=0.58cm, inner sep=3pt, align=center},
    arrow/.style={-{Latex[length=2.8mm,width=1.9mm]}, line width=1.0pt, draw=black!82},
    softarrow/.style={-{Latex[length=2.1mm,width=1.4mm]}, line width=0.8pt, draw=black!62},
    note/.style={font=\sffamily\tiny, text=black!74, align=center}
]
\node[note, text=RoyalBlue!70!black] at (1.05,3.28) {prefix $\va$};
\node[token, fill=RoyalBlue!18, draw=RoyalBlue!72!black] (a1) at (0.22,2.92) {$a_1$};
\node[token, fill=RoyalBlue!18, draw=RoyalBlue!72!black] (a2) at (0.68,2.92) {$a_2$};
\node[token, fill=RoyalBlue!18, draw=RoyalBlue!72!black] (a3) at (1.14,2.92) {$a_3$};
\node[note] at (1.50,2.92) {$\cdots$};
\node[token, fill=RoyalBlue!18, draw=RoyalBlue!72!black] (a4) at (1.88,2.92) {$a_n$};

\node[note, text=RoyalBlue!70!black] at (1.05,2.28) {stored prefix cache};
\node[slot, fill=RoyalBlue!12, draw=RoyalBlue!70!black] (pkv1) at (0.20,1.80) {$K,V$};
\node[slot, fill=RoyalBlue!12, draw=RoyalBlue!70!black] (pkv2) at (0.76,1.80) {$K,V$};
\node[slot, fill=RoyalBlue!12, draw=RoyalBlue!70!black] (pkv3) at (1.32,1.80) {$K,V$};
\node[note] at (1.74,1.80) {$\cdots$};
\node[slot, fill=RoyalBlue!12, draw=RoyalBlue!70!black] (pkv4) at (2.16,1.80) {$K,V$};

\node[block, fill=BurntOrange!20, draw=BurntOrange!85!black] (policy) at (3.25,1.80) {$\cl_\ell$};
\draw[arrow] (pkv4.east) -- (policy.west);
\node[note, text=BurntOrange!82!black] at (2.72,2.08) {replace};

\node[note, text=ForestGreen!58!black] at (4.88,2.20) {compressed prefix cache};
\node[slot, fill=ForestGreen!18, draw=ForestGreen!75!black] (ckv1) at (4.46,1.80) {$\tilde K,\tilde V$};
\node[slot, fill=ForestGreen!18, draw=ForestGreen!75!black] (ckv2) at (5.24,1.80) {$\tilde K,\tilde V$};
\node[note] at (4.86,1.36) {$\length(n) \le n$ slots};
\draw[arrow] (policy.east) -- (ckv1.west);

\node[note, text=Plum!72!black] at (1.05,0.92) {suffix $\vb$};
\node[token, fill=Plum!14, draw=Plum!72!black] (b1) at (0.32,0.52) {$b_1$};
\node[token, fill=Plum!14, draw=Plum!72!black] (b2) at (0.82,0.52) {$b_2$};
\node[note] at (1.22,0.52) {$\cdots$};
\node[token, fill=Plum!14, draw=Plum!72!black] (b3) at (1.62,0.52) {$b_k$};

\node[slot, fill=Plum!12, draw=Plum!72!black] (skv1) at (3.48,0.52) {$K',V'$};
\node[slot, fill=Plum!12, draw=Plum!72!black] (skv2) at (4.16,0.52) {$K',V'$};
\node[note] at (3.82,0.10) {ordinary suffix cache};
\draw[softarrow] (b3.east) -- (skv1.west);
\node[note, text=Plum!72!black] at (2.62,0.82) {compute normally};

\node[block, fill=Gray!14, draw=black!78, minimum width=1.32cm, minimum height=0.84cm] (attn) at (6.44,1.14) {suffix\\attention};
\draw[arrow, draw=ForestGreen!72!black] (ckv2.east) -- (attn.north west);
\draw[arrow, draw=Plum!72!black] (skv2.east) -- (attn.south west);
\node[note, anchor=west, text=ForestGreen!55!black] at (5.78,2.56) {only prefix\\slots shrink};
\end{tikzpicture}%


==> tikz/train_for_compressibility.tex <==
\begin{tikzpicture}[
    >=Latex,
    font=\sffamily\scriptsize,
    stage/.style={draw=black!78, line width=0.7pt, rounded corners=1.5pt, minimum width=1.18cm, minimum height=0.62cm, align=center, inner sep=3pt},
    result/.style={stage, minimum width=1.24cm, minimum height=0.78cm},
    cache/.style={draw=black!75, line width=0.55pt, rounded corners=1pt, minimum width=0.26cm, minimum height=0.42cm, inner sep=0pt},
    arrow/.style={-{Latex[length=3.0mm,width=2.0mm]}, line width=1.05pt, draw=black!82},
    note/.style={font=\sffamily\tiny, text=black!76, align=center},
    lane/.style={draw=black!18, line width=0.55pt, rounded corners=2pt, fill=black!2}
]
\node[lane, minimum width=7.25cm, minimum height=1.35cm, fill=RoyalBlue!4] at (3.62,2.72) {};
\node[lane, minimum width=7.25cm, minimum height=1.35cm, fill=ForestGreen!5] at (3.62,1.05) {};

\node[note, anchor=west, text=black!86] at (0.18,3.27) {\textbf{standard}};
\node[stage, fill=RoyalBlue!18, draw=RoyalBlue!72!black] (base) at (1.08,2.70) {fixed\\model};
\foreach \i/\x in {1/2.05,2/2.38,3/2.71,4/3.04,5/3.37,6/3.70}
    \node[cache, fill=RoyalBlue!22, draw=RoyalBlue!70!black] (b\i) at (\x,2.70) {};
\node[note, text=RoyalBlue!65!black] at (2.88,3.15) {dense target};
\node[stage, fill=BurntOrange!20, draw=BurntOrange!85!black, minimum width=1.38cm] (compA) at (4.88,2.70) {post-hoc\\compressor};
\node[result, fill=RedOrange!18, draw=RedOrange!85!black] (outA) at (6.48,2.70) {compact\\cache};
\draw[arrow] (base.east) -- (b1.west);
\draw[arrow] (b6.east) -- (compA.west);
\draw[arrow] (compA.east) -- (outA.west);

\node[note, anchor=west, text=black!86] at (0.18,1.60) {\textbf{this work}};
\node[stage, fill=ForestGreen!18, draw=ForestGreen!72!black] (train) at (1.08,1.03) {continued\\pretraining};
\node[stage, fill=Plum!18, draw=Plum!72!black, minimum width=0.94cm] (budget) at (2.40,1.03) {KV\\budget};
\foreach \i/\x in {1/3.20,2/3.53,3/3.86}
    \node[cache, fill=ForestGreen!28, draw=ForestGreen!75!black] (o\i) at (\x,1.03) {};
\node[note, text=ForestGreen!58!black] at (3.52,1.47) {compressible target};
\node[stage, fill=BurntOrange!20, draw=BurntOrange!85!black, minimum width=1.38cm] (compB) at (4.88,1.03) {post-hoc\\compressor};
\node[result, fill=ForestGreen!20, draw=ForestGreen!78!black] (outB) at (6.48,1.03) {compact\\cache};
\draw[arrow] (train.east) -- (budget.west);
\draw[arrow] (budget.east) -- (o1.west);
\draw[arrow] (o3.east) -- (compB.west);
\draw[arrow] (compB.east) -- (outB.west);
\end{tikzpicture}%

